Towards Automated Cyber Range Design: Characterizing and Matching Demands to Supplies

Cyber ranges mimic real-world cyber environments and are in high demand. Before building their own cyber ranges, organizations need to deeply understand what construction supplies are available to them. A fundamental supply is the cyber range architecture, which prompts an important research question: Which cyber range architecture is most appropriate for an organization's requirements? To answer this question, we propose an innovative framework to specify cyber range requirements, characterize cyber range architectures (based on our analysis of 45 cyber range architectures), and match cyber range architectures to cyber range requirements.

==> references_backup.tex <==
@article{yamin2020cyber,
  title={Cyber ranges and security testbeds: Scenarios, functions, tools and architecture},
  author={Yamin, Muhammad Mudassar and Katt, Basel and Gkioulos, Vasileios},
  journal={Computers \& Security},
  volume={88},
  pages={101636},
  year={2020},
  publisher={Elsevier}
}

@book{priyadarshini2018features,
  title={Features and architecture of the modern cyber range: a qualitative analysis and survey},
  author={Priyadarshini, Ishaani},
  year={2018},
  publisher={University of Delaware}
}

@article{ukwandu2020review,
  title={A review of cyber-ranges and test-beds: Current and future trends},
  author={Ukwandu, Elochukwu and Farah, Mohamed Amine Ben and Hindy, Hanan and Brosset, David and Kavallieros, Dimitris and Atkinson, Robert and Tachtatzis, Christos and Bures, Miroslav and Andonovic, Ivan and Bellekens, Xavier},
  journal={Sensors},
  volume={20},
  number={24},
  pages={7148},
  year={2020},
  publisher={MDPI}
}

@article{chouliaras2021cyber,
  title={Cyber ranges and testbeds for education, training, and research},
  author={Chouliaras, Nestoras and Kittes, George and Kantzavelou, Ioanna and Maglaras, Leandros and Pantziou, Grammati and Ferrag, Mohamed Amine},
  journal={Applied Sciences},
  volume={11},
  number={4},
  pages={1809},
  year={2021},
  publisher={MDPI}
}

@article{davis2013survey,
  title={A survey of cyber ranges and testbeds},
  author={Davis, Jon and Magrath, Shane},
  year={2013},
  publisher={DEFENCE SCIENCE AND TECHNOLOGY ORGANISATION EDINBURGH (AUSTRALIA) CYBER AND~…}
}

@article{Or-Meir2019Dynamic,
author = {Or-Meir, Ori and Nissim, Nir and Elovici, Yuval and Rokach, Lior},
title = {Dynamic Malware Analysis in the Modern Era—A State of the Art Survey},
year = {2019},
issue_date = {September 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {52},
number = {5},
issn = {0360-0300},
url = {https://doi-org.libproxy.uccs.edu/10.1145/3329786},
doi = {10.1145/3329786},
abstract = {Although malicious software (malware) has been around since the early days of computers, the sophistication and innovation of malware has increased over the years. In particular, the latest crop of ransomware has drawn attention to the dangers of malicious software, which can cause harm to private users as well as corporations, public services (hospitals and transportation systems), governments, and security institutions. To protect these institutions and the public from malware attacks, malicious activity must be detected as early as possible, preferably before it conducts its harmful acts. However, it is not always easy to know what to look for—especially when dealing with new and unknown malware that has never been seen. Analyzing a suspicious file by static or dynamic analysis methods can provide relevant and valuable information regarding a file's impact on the hosting system and help determine whether the file is malicious or not, based on the method's predefined rules. While various techniques (e.g., code obfuscation, dynamic code loading, encryption, and packing) can be used by malware writers to evade static analysis (including signature-based anti-virus tools), dynamic analysis is robust to these techniques and can provide greater understanding regarding the analyzed file and consequently can lead to better detection capabilities. Although dynamic analysis is more robust than static analysis, existing dynamic analysis tools and techniques are imperfect, and there is no single tool that can cover all aspects of malware behavior. The most recent comprehensive survey performed in this area was published in 2012. Since that time, the computing environment has changed dramatically with new types of malware (ransomware, cryptominers), new analysis methods (volatile memory forensics, side-channel analysis), new computing environments (cloud computing, IoT devices), new machine-learning algorithms, and more. The goal of this survey is to provide a comprehensive and up-to-date overview of existing methods used to dynamically analyze malware, which includes a description of each method, its strengths and weaknesses, and its resilience against malware evasion techniques. In addition, we include an overview of prominent studies presenting the usage of machine-learning methods to enhance dynamic malware analysis capabilities aimed at detection, classification, and categorization.},
journal = {ACM Comput. Surv.},
month = {sep},
articleno = {88},
numpages = {48},
keywords = {Dynamic analysis, detection, evasion, malware, behavioral analysis}
}

@inproceedings{levin2003lessons,
  title={Lessons learned in using live red teams in IA experiments},
  author={Levin, David},
  booktitle={Proceedings DARPA Information Survivability Conference and Exposition},
  volume={1},
  pages={110--119},
  year={2003},
  organization={IEEE}
}

@inproceedings{luise2021demand,
  title={On-demand Deployment and Orchestration of Cyber Ranges in the Cloud.},
  author={Luise, Alessandro Placido and Perrone, Gaetano and Perrotta, Claudio and Romano, Simon Pietro},
  booktitle={ITASEC},
  pages={80--91},
  year={2021}
}

@article{mirkovic2012teaching,
  title={Teaching cybersecurity with DeterLab},
  author={Mirkovic, Jelena and Benzel, Terry},
  journal={IEEE Security \& Privacy},
  volume={10},
  number={1},
  pages={73--76},
  year={2012},
  publisher={IEEE}
}

@article{kucek2020empirical,
  title={An empirical survey of functions and configurations of open-source capture the flag (CTF) environments},
  author={Kucek, Stela and Leitner, Maria},
  journal={Journal of Network and Computer Applications},
  volume={151},
  pages={102470},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{beuran2022aws,
  title={AWS EC2 Public Cloud Cyber Range Deployment},
  author={Beuran, Razvan and Zhang, Zhe and Tan, Yasuo},
  booktitle={2022 IEEE European Symposium on Security and Privacy Workshops (EuroS\&PW)},
  pages={433--441},
  year={2022},
  organization={IEEE}
}

@inproceedings{orbinato2021next,
  title={A next-generation platform for Cyber Range-as-a-Service},
  author={Orbinato, Vittorio},
  booktitle={2021 IEEE International Symposium on Software Reliability Engineering Workshops (ISSREW)},
  pages={314--318},
  year={2021},
  organization={IEEE}
}

@article{farhat2021design,
  title={Design and Development of the Back-End Software Architecture for a Hybrid Cyber Range},
  author={Farhat, Hussein},
  year={2021}
}

@inproceedings{macak2022applying,
  title={Applying Process Discovery to Cybersecurity Training: An Experience Report},
  author={Macak, Martin and Oslejsek, Radek and Buhnova, Barbora},
  booktitle={2022 IEEE European Symposium on Security and Privacy Workshops (EuroS\&PW)},
  pages={394--402},
  year={2022},
  organization={IEEE}
}

@inproceedings{vykopal2021scalable,
  title={Scalable learning environments for teaching cybersecurity hands-on},
  author={Vykopal, Jan and {\v{C}}eleda, Pavel and Seda, Pavel and {\v{S}}v{\'a}bensk{\`y}, Valdemar and Tovar{\v{n}}{\'a}k, Daniel},
  booktitle={2021 IEEE Frontiers in Education Conference (FIE)},
  pages={1--9},
  year={2021},
  organization={IEEE}
}

@inproceedings{debatty2019building,
  title={Building a cyber range for training cyberdefense situation awareness},
  author={Debatty, Thibault and Mees, Wim},
  booktitle={2019 International Conference on Military Communications and Information Systems (ICMCIS},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@article{bridges2022testing,
  title={Testing SOAR Tools in Use},
  author={Bridges, Robert A and Rice, Ashley E and Oesch, Sean and Nichols, Jeff A and Watson, Cory and Spakes, Kevin and Norem, Savannah and Huettel, Mike and Jewell, Brian and Weber, Brian and others},
  journal={arXiv preprint arXiv:2208.06075},
  year={2022}
}

@inproceedings{vielberth2021digital,
  title={A digital twin-based cyber range for SOC analysts},
  author={Vielberth, Manfred and Glas, Magdalena and Dietz, Marietheres and Karagiannis, Stylianos and Magkos, Emmanouil and Pernul, G{\"u}nther},
  booktitle={IFIP Annual Conference on Data and Applications Security and Privacy},
  pages={293--311},
  year={2021},
  organization={Springer}
}


@article{Rockeman_hackers_2022,
	title = {Hackers’ Path Eased as 600,000 {U.S.} Cybersecurity Jobs Sit Empty},
        author = {Rockeman, Olivia},
	url = {https://www.bloomberg.com/news/articles/2022-03-30/hackers-path-is-eased-as-600-000-cybersecurity-jobs-sit-empty},
	abstract = {President Joe Biden has urged U.S. companies to “harden your cyber defenses immediately” amid a growing risk of Russian cyberattacks. For many, that won’t be easy.},
	journaltitle = {Bloomberg.com},
	urldate = {2022-12-15},
	date = {2022-03-30},
	langid = {english},
	keywords = {business, cybersecurity, Cybersecurity, Homeland Security, Jobs, Joe Biden, Labor, politics, Software, technology, War},
}

@inproceedings{hermenier2012build,
  title={How to build a better testbed: Lessons from a decade of network experiments on emulab},
  author={Hermenier, Fabien and Ricci, Robert},
  booktitle={International Conference on Testbeds and Research Infrastructures},
  pages={287--304},
  year={2012},
  organization={Springer}
}

@online{VirginiaTech_uscyberrange,
	title = {{U.S. Cyber Range}},
    author = {{Virginia Tech}},
	url = {https://uscyberrange.org},
	abstract = {Scalable, cloud-hosted infrastructure providing students with virtual environments for realistic, hands-on cybersecurity labs and exercises.},
	urldate = {2022-12-15},
	langid = {english},
	file = {Snapshot:C\:\\Users\\ekzhi\\Zotero\\storage\\842I2PSA\\www.uscyberrange.org.html:text/html},
}


@online{cyberventure_cybercrime_2020,
	title = {Cybercrime To Cost The World \$10.5 Trillion Annually By 2025},
	url = {https://cybersecurityventures.com/hackerpocalypse-cybercrime-report-2016/},
	abstract = {Special Report: Cyberwarfare In The C-Suite.},
	titleaddon = {Cybercrime Magazine},
	author = {{Cybercrime Magazine}},
	urldate = {2022-12-15},
	date = {2020-11-13},
	langid = {american},
	note = {Section: Reports},
	file = {Snapshot:C\:\\Users\\ekzhi\\Zotero\\storage\\MQMNQWIX\\hackerpocalypse-cybercrime-report-2016.html:text/html},
}

@article{pernik_improving_2014,
	title = {Improving Cyber Security: {NATO} and the {EU}},
	author = {Pernik, Piret},
	langid = {english},
        year = {2014},
	file = {Pernik - Improving Cyber Security NATO and the EU.pdf:C\:\\Users\\ekzhi\\Zotero\\storage\\JASVLH98\\Pernik - Improving Cyber Security NATO and the EU.pdf:application/pdf},
}


@online{qiu_cisco_2015,
	title = {Cisco Cyber Range},
	url = {https://www.cisco.com/c/dam/global/en_hk/assets/event/cisco_connect_2015/pdf/4-3.pdf},
	author = {Qiu, Paul},
	urldate = {2022-12-15},
	date = {2015},
	file = {4-3.pdf:C\:\\Users\\ekzhi\\Zotero\\storage\\SKJHITRR\\4-3.pdf:application/pdf},
}

@book{deane2021official,
  title={The Official (ISC) 2 CISSP CBK Reference},
  author={Deane, Arthur J and Kraus, Aaron},
  year={2021},
  publisher={John Wiley \& Sons}
}

@article{beuran2018integrated,
  title={Integrated framework for hands-on cybersecurity training: CyTrONE},
  author={Beuran, Razvan and Tang, Dat and Pham, Cuong and Chinen, Ken-ichi and Tan, Yasuo and Shinoda, Yoichi},
  journal={Computers \& Security},
  volume={78},
  pages={43--59},
  year={2018},
  publisher={Elsevier}
}


@phdthesis{karagiannis2022systematic,
  title={Systematic Design, Deployment and Evaluation of Gamified Cybersecurity Learning Environments},
  author={Karagiannis, Stylianos},
  year={2022},
  school={I{\'o}$\nu$$\iota$o $\Pi$$\alpha$$\nu$$\varepsilon$$\pi$$\iota$$\sigma$$\tau$$\acute{\eta}$$\mu$$\iota$o. $\Sigma$$\chi$o$\lambda$$\acute{\eta}$ E$\pi$$\iota$$\sigma$$\tau$$\acute{\eta}$$\mu$$\eta$$\varsigma$ $\tau$$\eta$$\varsigma$ $\Pi$$\lambda$$\eta$$\rho$o$\varphi$o$\rho$$\acute{\iota}$$\alpha$$\varsigma$ $\kappa$$\alpha$$\iota$ $\Pi$$\lambda$$\eta$$\rho$o$\varphi$o$\rho$$\iota$$\kappa$$\acute{\eta}$$\varsigma$. T$\mu$$\acute{\eta}$$\mu$$\alpha$~…}
}

@inproceedings{potamos2021towards,
  title={Towards a maritime cyber range training environment},
  author={Potamos, Georgios and Peratikou, Adamantini and Stavrou, Stavros},
  booktitle={2021 IEEE International Conference on Cyber Security and Resilience (CSR)},
  pages={180--185},
  year={2021},
  organization={IEEE}
}

@article{ahmad2021design,
  title={Design and Implementation of a network of specialized and Hybrid Cyber-Ranges},
  author={Ahmad, Shabeer and others},
  year={2021},
  publisher={Gran Sasso Science Institute}
}

@inproceedings{coshatt2022design,
  title={Design of Cyber-Physical Security Testbed for Multi-Stage Manufacturing System},
  author={Coshatt, Stephen J and Li, Qi and Yang, Bowen and Wu, Shushan and Shrivastava, Darpan and Ye, Jin and Song, WenZhan and Zahiri, Feraidoon},
  booktitle={GLOBECOM 2022-2022 IEEE Global Communications Conference},
  pages={1978--1983},
  year={2022},
  organization={IEEE}
}

@inproceedings{ronkainen2012mtt,
  title={MTT CropInfra},
  author={Ronkainen, Ari and Teye, Frederick and Koistinen, Markku and Kaivosoja, Jere and Pesonen, Liisa and Suomi, Pasi},
  booktitle={Testbeds and Research Infrastructure. Development of Networks and Communities: ICST},
  year={2012},
  organization={Springer}
}

@inproceedings{luglio2012satellite,
  title={A satellite network emulation platform for implementation and testing of TCP/IP applications},
  author={Luglio, Michele and Roseti, Cesare and Zampgnaro, Francesco},
  booktitle={Testbeds and Research Infrastructure. Development of Networks and Communities: ICST},
  pages={1--2},
  year={2012},
  organization={Springer}
}

@inproceedings{virag2021current,
  title={The current state of the art and future of European Cyber Range Ecosystem},
  author={Vir{\'a}g, Csaba and {\v{C}}egan, Jakub and Lieskovan, Tom{\'a}{\v{s}} and Merialdo, Matteo},
  booktitle={2021 IEEE International Conference on Cyber Security and Resilience (CSR)},
  pages={390--395},
  year={2021},
  organization={IEEE}
}

@article{hogan2011nist,
  title={Nist cloud computing standards roadmap},
  author={Hogan, Michael and Liu, Fang and Sokol, Annie and Tong, Jin},
  journal={NIST Special Publication},
  volume={35},
  pages={6--11},
  year={2011}
}

@article{beuran2023capability,
  title={Capability Assessment Methodology and Comparative Analysis of Cybersecurity Training Platforms},
  author={Beuran, Razvan and Vykopal, Jan and Belajov{\'a}, Daniela and {\v{C}}eleda, Pavel and Tan, Yasuo and Shinoda, Yoichi},
  journal={Computers \& Security},
  pages={103120},
  year={2023},
  publisher={Elsevier}
}

@article{mogull2021security,
  title={Security guidance for critical areas of focus in cloud computing v4.0},
  author={Mogull, Rich and Arlen, J and Gilbert, F and Lane, A and Mortman, D and Peterson, G and Rothman, M and Moltz, J and Moren, D and Scoboria, E},
  journal={Cloud Security Alliance},
  year={2021}
}

@article{batterton2017likert,
  title={The Likert scale what it is and how to use it},
  author={Batterton, Katherine A and Hale, Kimberly N},
  journal={Phalanx},
  volume={50},
  number={2},
  pages={32--39},
  year={2017},
  publisher={JSTOR}
}

@inproceedings{lieskovan2021building,
  title={Building Open Source Cyber Range To Teach Cyber Security},
  author={Lieskovan, Tomas and Hajn{\`y}, Jan},
  booktitle={Proceedings of the 16th International Conference on Availability, Reliability and Security},
  pages={1--11},
  year={2021}
}

@inproceedings{smeets2022role,
  title={The role of military cyber exercises: A case study of locked shields},
  author={Smeets, Max},
  booktitle={2022 14th International Conference on Cyber Conflict: Keep Moving!(CyCon)},
  volume={700},
  pages={9--25},
  year={2022},
  organization={IEEE}
}

@article{tian2018real,
  title={A real-time correlation of host-level events in cyber range service for smart campus},
  author={Tian, Zhihong and Cui, Yu and An, Lun and Su, Shen and Yin, Xiaoxia and Yin, Lihua and Cui, Xiang},
  journal={IEEE Access},
  volume={6},
  pages={35355--35364},
  year={2018},
  publisher={IEEE}
}
